Quasi Normality and PL Approximation of Least Area Surfaces in 3-Manifolds

This} paper presents relations between least area and normal surfaces, embedded in either a Euclidean or hyperbolic $3$-manifold. A relaxed version of normal surfaces, termed quasi-normal, is introduced, and it is shown that under appropriate conditions, every embedded least area surface is quasi-normal with respect to a fine enough fat triangulation of the $3$-manifold. In addition, it is shown that the intersections of a least area surface with the tetrahedra of such fine enough triangulation, even when not as simple as in the case of normal surfaces, are also well behaved. Finally, it is shown that a least area surface, when considered as a quasi normal surface, gives rise to a sequence of piecewise flat surfaces termed as flat-associated surfaces, and this sequence converges to the given least area surface and approximates its area.

==> QuasiNormalAppxThmQuasiBoundary.tex <==
\section{Manifolds with Boundary}
This section generalizes Theorems \ref{thm:LeastAreaIsNormal} and \ref{thm:NonNormalAreTame} to compact $3$-manifolds with boundary. Doing so requires some modifications in the proofs of those theorems which will be given herein. Before stating the generalized theorem a care need be taken for the mere existence of least area surfaces in manifolds with boundary. For that, the route taken in ~\cite{hs} will be followed. 
\begin{df}
A Riemannian three manifold $\mcal{M}$ has {\emph sufficiently convex} boundary if:
\begin{enum}
 \item $\del \mcal{M}$ is piecewise smooth.
 \item Each smooth subsurface of $\del \mcal{M}$ has non-negative mean curvature with respect to the inward normal.
 \item There exists a Riemannian three manifold $\mcal{N}$ such that $\mcal{M}$ is isometric to a submanifold of $\mcal{N}$, and each smooth subsurface $\mcal{S}$ of $\del \mcal{M}$ extends to a smooth subsurface $\mcal{S}'$ embedded in $\mcal{N}$ such that $\mcal{S}' \cap \mcal{M} = \mcal{S}$.
\end{enum}
\end{df} 
\noindent{Further}, the following definition given by Morrey in ~\cite{morr} is necessary in order to assure the existence of the curvature and injectivity radius bounds that are used in the proofs of Theorems  \ref{thm:LeastAreaIsNormal} and \ref{thm:NonNormalAreTame}.
\begin{df}
A Riemnnian three manifold is {\emph homogeneously regular} if there exist positive constants $k, K$ so that every point of the manifolds lies in the image of a chart $\varphi$ with domain the unit ball $B(0, 1)$ in $\mathbb{R}^3$ such that \[ k||\nu||^2 \leq g_{ij}(\varphi (x))\nu_i \nu_j \leq K||\nu||^2\] for all $x \in B(0, 1)$,
where $\nu$ is any tangent vector to $x$, and $g_{ij}$ are the components of the metric $g$ on $\mcal{M}$.
\end{df}
In ~\cite{my3} existence and uniqueness of least area disks spanned by simple closed curves in the boundary of a three manifold with sufficiently convex boundary are proven, see also ~\cite{hs}, Section $6$. In addition, Lemmas ~\ref{lem:DiskSpanCurve} and ~\ref{lem:ShortEnoughCurve} extend to homogeneously regular three manifolds with sufficiently convex boundary, see Section $6$ of ~\cite{hs}. Note that if $\mcal{T}$ is a triangulation of a three-manifold with boundary then $\mcal{T}$ induces a triangulation of $\partial \mcal{M}$, and according to ~\cite{hs} if $\mcal{M}$ is homogeneously regular with sufficiently convex boundary then the boundary of small enough $2$-face of $\mcal{T}$ that is embedded in $\partial \mcal{M}$ bounds a least area disk in $\mcal{M}$, that is either properly embedded in $\mcal{M}$ or a subset of $\partial \mcal{M}$. In the proof of Lemma \ref{lem:NoSimpleClosedCurves} we used the fact that $\mcal{T}$ is a least area triangulation, so every $2$-face is a least area disk. This assumption may not hold for three manifolds with boundary, for example in the case where a least area disk bounded by a simple closed curve included in $\partial \mcal{M}$ is properly embedded in $\mcal{M}$. 
As a result a proper modification of Theorem \ref{thm:LeastAreaIsNormal} needs to be stated. 
Before stating the appropriate theorem the following definition is required.
\begin{df}
Let $\mcal{T}$ be a triangulation of a three manifold with boundary. A $2$-face of $\mcal{T}$ is called {\emph peripheral} if it has non empty intersection with $\partial \mcal{M}$. A $2$-face is called {\emph boundary $2$-face} if it is embedded in $\partial \mcal{M}$. A triangulation is called {\emph internally least area} if every $2$-face that is not a boundary $2$-face is a least area disk spanned by its boundary.
\end{df}
\noindent{In} order to simplify the statement of the following theorem the definition of quasi-normal surface is altered.
\begin{df}
A surface $(\mcal{F}, \partial \mcal{F})$ properly embedded in a triangulated three manifold $(\mcal{M}, \partial \mcal{M}, \mcal{T})$ is {\emph internally quasi-normal} if its non-normal intersection with $\mcal{T}$ are bent curves, and a (possibly empty) collection of simple closed curves, each is contained in a boundary $2$-face of $\mcal{T}$, and bounds a least area disk properly embedded in a peripheral tetrahedron of $\mcal{T}$.
\end{df} 
\noindent{With} these definitions  at hand Theorem \ref{thm:LeastAreaIsNormal} is restated as follows:

\renewcommand{\thethm}{\arabic{thm}}%{\Alph{thm}}
\setcounter{thm}{2}
\begin{thm} \label{thm:LeastAreaQuasiNormalBoundary}
Let $\mcal{M}$ be an irreducible, orientable, homogeneously regular Euclidean or hyperbolic three manifold with sufficiently convex boundary. Let $\mcal{F}$ be a two-sided incompressible, $\partial$-incompressible, least area surface properly embedded in $\mcal{M}$. Let $\mcal{T}$ be some geodesic internally least area triangulation of $\mcal{M}$, so that $\mcal{F} \cap \mcal{T}^{(0)} = \emptyset$. Then for every $0 < \varphi < \frac{\pi}{2}$ there exists a constant $\Psi > 0$ that depends only on $inj_{\mcal{M}}, K_{\mcal{M}}$, and $\varphi$, such that if $\mcal{T}$ is $\varphi$-fat, and $\lambda(\mcal{T}) < \Psi$, then $\mcal{F}$ is internally quasi-normal with respect to $\mcal{T}$.
\end{thm}
\renewcommand{\thethm}{\thesection.\arabic{thm}}
\setcounter{thm}{1}
In order to prove Theorem \ref{thm:LeastAreaQuasiNormalBoundary} Lemma \ref{lem:NoSimpleClosedCurves} becomes the following lemma which in a sense resembles Lemma $6.7$ of ~\cite{hs}:
\begin{lem} \label{lem:NoSimpleClosedCurvesBoundary}
There exists $\epsilon > 0$ such that if $\mcal{T}$ is $\varphi$-fat for some positive $\varphi$, and $\lambda(\mcal{T}) < \epsilon$ then the intersection of $\mcal{F}$ with the interior of any $2$-faces of $\mcal{T}$ that is not a boundary $2$-face does not contain simple closed curves, and if $\gamma \in \partial \mcal{F}$ is a simple closed curve contained in the interior of a boundary $2$-face of $\mcal{T}$ then $\gamma$ bounds a least area disk that is either contained in $\partial \mcal{M}$ or properly embedded in $mcal{M}$ 
\end{lem}
\begin{proof}
Let $\frak{f}$ be a $2$-face of $\mcal{T}$. If $\frak{f}$ is not a boundary $2$-face then all arguments in the proof of Lemma ~\ref{lem:NoSimpleClosedCurves} hold, so the proof is identical. Suppose $\frak{f}$ is a boundary $2$-face, and that $\gamma \in \partial \mcal{F}$ is a simple closed curve contained in the interior of $\frak{f}$. Let $\mcal{N} = \mcal{N}(\delta, \gamma, \mcal{F})$ be a $\delta$-collar neighborhood of $\gamma$ in $\mcal{F}$, for some small enough $\delta$ so that $ \mcal{N}$ is entirely contained in a tetrahedron $\tau \in \mcal{T}$ of which $\frak{f}$ is a $2$-face. Let $\Gamma \in \partial \mcal{N}$ be the parallel of $\gamma$ in the boundary of $\mcal{N}$. Then $\Gamma$ is a simple closed curve in $\mcal{F}$ contained in the $3$-ball $\tau$, and since $\mcal{F}$ is incompressible $\Gamma$ bounds a disk $\mcal{D}$ in $\mcal{F}$. As a result $\gamma$ is the boundary of a disk $\mcal{E} = \mcal{D} \cup \mcal{N}$ that is contained in $\mcal{F}$. If the disk $\mcal{D}$ is not entirely contained in $\tau$ then the situation is identical to case II of the proof of Lemma ~\ref{lem:NoSimpleClosedCurves}, and the arguments used in this case still hold, so the proof proceeds identically. If $\mcal{D}$ is contained in $\tau$ then the interior of $\mcal{E}$ is contained in $\tau$ as well. In addition, $\gamma$ bounds a disk $\mcal{D}'$ in the $2$-face $\frak{f}$. Since $\mcal{F}$ is embedded in $\mcal{M}$, the disk $\mcal{D}$ is embedded, and as a result $\mcal{E}$ is embedded as well. Hence, $\mcal{D}' \cup \mcal{E}$ is a $2$-sphere embedded in $\mcal{M}$. Therefore, since $\mcal{M}$ is irreducible the disk $\mcal{E}$ there is an isotopy of $\mcal{F}$ mapping $\mcal{E}$ isotopically to $\mcal{D}'$, and which is the identity elsewhere. If this isotopy reduces the area of $\mcal{F}$ then the disk $\mcal{D}'$ is a least area disk bounded by $\gamma$, otherwise, according to lemma $6.6$ of ~\cite{hs} $\gamma$ bounds least area disk that is properly embedded in the tetrahedron $\tau$ which, by definition, is a peripheral tetrahedron, and the proof of the lemma is completed.
\end{proof}
\noindent{The} following two lemmas are the appropriate versions of Lemmas \ref{lem:IntesectionsAreDisks}, and \ref{lem:3Or4Gon} for the case $\mcal{M}$ has non-empty boundary.
\begin{lem}\label{lem:IntesectionsAreDisksBoundary}
Let $\mcal{M}$ be homogeneously regular three manifold with sufficiently convex boundary. There exists $\epsilon > 0$ such that if $\lambda(\mcal{T}) < \epsilon$, then the intersection of $\mcal{F}$ with any tetrahedron of $\mcal{T}$ is a (possibly empty) collection of disks.
\end{lem}

\begin{lem}\label{lem:3Or4GonBoundary}
Let $\mcal{M}$ be homogeneously regular three manifold with sufficiently convex boundary. For every $0 < \varphi < \frac{\pi}{2}$ there exists $\epsilon > 0$ that depends only on $inj_{\mcal{M}}, K_{\mcal{M}}$ and $\varphi$, such that if $\lambda(\mcal{T}) < \epsilon$, and $\mcal{T}$ is $\varphi$-fat, then every normal disk in $\mcal{F} \cap \mcal{T}$ is either a $3$-gon or a $4$-gon.
\end{lem}
\noindent{Since} the proofs of both Lemmas \ref{lem:IntesectionsAreDisks}, and \ref{lem:3Or4Gon} heavily relies on the curvature bound of Schoen, and since, according to \cite{morr} being homogeneously regular is equivalent to having global bound on the curvature in the case of three manifold with boundary, the proof of Lemma \ref{lem:IntesectionsAreDisksBoundary} remains the same as the proof of Lemma \ref{lem:IntesectionsAreDisks}, and the proof of Lemma \ref{lem:3Or4GonBoundary} is identical to that of \ref{lem:3Or4Gon}. 
One thing to notice however, is the following:

\begin{rem}\label{rem:NoPeripheralBentCurves}
If $\frak{f}$ is a peripheral $2$-face that is not a boundary $2$-face, so that $\frak{f}$ meets $\partial \mcal{M}$ transversally along an edge $e$, then there cannot be any bent curve in $\frak{f}$ having both end points on $e$. 
This is because the surface $\mcal{F}$ is $\partial$-incompressible in $\mcal{M}$, and any such bent curve gives rise to $\partial$-compression. 
\end{rem}

\noindent{The} proof of Theorem \ref{thm:LeastAreaQuasiNormalBoundary} follows from Lemmas \ref{lem:NoSimpleClosedCurvesBoundary}, \ref{lem:IntesectionsAreDisksBoundary}, and \ref{lem:3Or4GonBoundary} exactly the same way as Theorem \ref{thm:LeastAreaIsNormal} follows from Lemmas \ref{lem:NoSimpleClosedCurves}, \ref{lem:IntesectionsAreDisks}, and \ref{lem:3Or4Gon}

\renewcommand{\thethm}{\arabic{thm}}%{\Alph{thm}}
\setcounter{thm}{3}
\begin{thm}\label{thm:NonNormalAreTameBoundary}
Let $\mcal{F}$ be an incompressible, $\partial$-incompressible, $2$-sided least area surface in a homogeneously regular, irreducible, orientable hyperbolic or Euclidean $3$-manifold $\mcal{M}$, with sufficiently convex boundary. Let $\Psi$ be the constant obtained in Theorem \ref{thm:LeastAreaIsNormal}, and let $\mcal{T}$ be a geodesic, internally least area, $\varphi$-fat triangulation of $\mcal{M}$ so that $\lambda(\mcal{T}) < \Psi$ and $\mcal{F}$ quasi normal with respect to $\mcal{T}$. Then every non normal disk in $\mcal{F} \cap \mcal{T}^{(3)}$ can be presented as a graph of a function defined on a disk that is contained in a single $2$-face of $\mcal{T}$.
\end{thm}
\renewcommand{\thethm}{\thesection.\arabic{thm}}
\setcounter{thm}{1}
\begin{proof} 
The proof of the theorem is similar to the proof of Theorem \ref{thm:NonNormalAreTame} which completely relies on the existence of global bound on the curvature of stable minimal surfaces in a closed three manifold. Again, homogeneous regularity of the manifold imposes the existence of such bound. In light of Remark \ref{rem:NoPeripheralBentCurves} the proof is simplified as some possible cases are actually impossible and need not be considered.
\end{proof}


